Structured Uncertainty Prediction Networks

This paper is the first work to propose a network to predict a structured uncertainty distribution for a synthesized image. Previous approaches have been mostly limited to predicting diagonal covariance matrices. Our novel model learns to predict a full Gaussian covariance matrix for each reconstruction, which permits efficient sampling and likelihood evaluation. We demonstrate that our model can accurately reconstruct ground truth correlated residual distributions for synthetic datasets and generate plausible high frequency samples for real face images. We also illustrate the use of these predicted covariances for structure preserving image denoising.

==> background.tex <==
\section{Background}

The VAE consists of (i) a decoder or generator model, $p_{\btheta}(\bx| \bz)$, which models the probability distribution of the input data $\bx$ conditioned on the low-dimensional representation $\bz$ in a latent space and (ii) an encoder or recognition model, $q_{\bphi}(\bz|\bx)$, which maps in the other direction. 
Both models are described using deep neural networks, with parameters $\btheta$ and $\bphi$ respectively.
During training the parameters are estimated such that the marginal likelihood of the training data, $p_{\btheta}(\bx)$, is maximized under a variational Bayesian approximation:
%\vspace{-0.1cm}
\begin{equation}
\log\left[p_{\btheta}(\bx)\right] = D_{KL}\left[q_{\bphi}(\bz|\bx)|| p_{\btheta}(\bz|\bx)\right] +  L_{VAE},
\label{eq:vae_intractable_loss}
\end{equation}%\vspace{-0.1cm}
\noindent where the variational lower bound is
%\vspace{-0.1cm}
\begin{equation}
\begin{split}
L_{VAE} &= \mathbb{E}_{q_{\bphi}(\bz|\bx)} \left[ \log ~ p_{\btheta}(\bx| \bz) \right] - \\
 & D_{KL}\left[q_{\bphi}(\bz|\bx)|| p_{\btheta}(\bz)\right].\\
\end{split}
\label{eq:vae-model}
\end{equation}

In the standard derivation of VAEs the decoder distribution is a multivariate Gaussian with diagonal covariance
\begin{equation}
 \log ~ p_{\btheta}(\bx|\bz) = \log \mathcal{N}(\boldsymbol{\mu}(\bz), \boldsymbol{\sigma}(\bz) \bI),
\end{equation}
where $\boldsymbol{\mu}$ and $\boldsymbol{\sigma}$ are functions of the latent code $\bz$.
In practice $\boldsymbol{\sigma}$ is never used to generate new data as it is quite a poor choice for a noise model, and it is only estimated to have the proper weighting in the loss.
In other words the output image of the VAE directly corresponds to the mean estimated by the network $\bhx = \boldsymbol{\mu}(\bz)$.
Moreover, it is common to assume that $\boldsymbol{\sigma}_i = \sigma$ is fixed to some user defined value.
Thus, the $\boldsymbol{\sigma}$ estimation is avoided altogether by assuming a shared variance, which simplifies the reconstruction loss to a sum of squared errors scaled by $\sigma$.


==> experiments_plan.tex <==
\section{Plan of experiments}
\begin{enumerate}
	\item Previous work
	\begin{enumerate}
		\item Variational Autoencoder
		\begin{enumerate}
			\item Original VAE~\cite{Kingma2014}$^*$
			\item Importance weighted autoencoders~\cite{Burda2016IWAE}$^\ddagger$ \href{https://github.com/yburda/iwae}{theano code}
			\item VAE with normalizing flow~\cite{Rezende2015NF}$^\ddagger$ Only third party implementations \href{https://github.com/casperkaae/parmesan}{theano}, \href{https://github.com/wellecks/vaes}{tf1}, \href{https://github.com/abhisheksaurabh1985/vae_nf}{tf2}
			\item VAE with Inverse Autoregressive Flow~\cite{Kingma2016IAF}$^\ddagger$ \href{https://github.com/openai/iaf}{tf code}
		\end{enumerate}
		\item GAN
		\begin{enumerate}
			\item DCGAN~\cite{Radford2016DCGAN}$^{*} ~^\dagger ~^\circ$
			\item BEGAN~\cite{Berthelot2017BEGAN} \href{https://github.com/carpedm20/BEGAN-tensorflow}{tf code}
			\item WGAN~\cite{Arjovsky2017WGAN}$^\dagger$ \href{https://github.com/martinarjovsky/WassersteinGAN}{pytorch code}
		\end{enumerate}
		\item Autoregressive models
		\begin{enumerate}
			\item PixelRNN~\cite{Oord2016PixelRNN}$^\dagger ~^\circ ~^\ddagger$ \href{https://github.com/carpedm20/pixel-rnn-tensorflow}{tf code}
			\item PixelCNN++~\cite{Salimans2017PixelCNNpp}$^\dagger ~^\circ$ \href{https://github.com/openai/pixel-cnn}{tf code}
		\end{enumerate}
		\item VAE/GAN
		\begin{enumerate}
			\item Adversarial Learned Inference~\cite{Dumoulin2016ALI}$^\dagger$ \href{https://github.com/IshmaelBelghazi/ALI}{theano code}
			\item Adversarial variational bayes~\cite{Mescheder2017AVB}$^\ddagger$ \href{https://github.com/LMescheder/AdversarialVariationalBayes}{tf code}
		\end{enumerate}
		\item Datasets
		\begin{enumerate}
			\item Custom toy dataset
			\item MNIST
			\item CIFAR-10
			\item CelebA
			\item Tiny Imagenet (64 $\times$ 64 images)
		\end{enumerate}
	\end{enumerate}
	\item Figures in the paper
	\begin{enumerate}
		\item Reconstructions from our method vs previous work
		\item Samples from our method
%		\item Fixed image and varying samples from $\bSigma$
%		\item Training loss vs number of samples from $\bSigma$
%		\item Real vs estimated $\bSigma$ for toy dataset
%		\item Comparison of modelling $\sigma\bI$ vs $\boldsymbol{\sigma}\bI$ vs $\bSigma$, or maybe just show samples from $\mathcal{N}(\mathbf{0}, \boldsymbol{\sigma}\bI)$
	\end{enumerate}
	\item Explicit matrix representation methods
	\begin{enumerate}
		\item Gamma diagonal prior and inverse Wishart
		\item Show reconstructions and samples for best method on toy dataset
%		\item Cholesky vs Eigen vs Eigen with diagonal
%		\item For Eigen the effect of changing the number of eigen vectors
%		\item For Eigen with diagonal, modelling $\bSigma$ vs $\bLambda$
	\end{enumerate}
	\item Black box method
	\begin{enumerate}
		\item Effect of each of the losses
		\item Train model with matrix of variable filters
		\begin{enumerate}
			\item Priors: diagonal on filters and smoothness on weights.
			Also figure in the paper with the effect of the priors.
			\begin{enumerate}
			\item Population prior
			\item Smoothness prior
			\item Diagonal prior, inverse square root Gamma
			\end{enumerate}			 
			\item Larger field of view for the filters with dilated convolutions, for the basis model, it might make sense to have some dense and some dilated convolutions.
%			\item Reduce number of parameters with symmetry constrains or interpolation between neighbouring pixels
		\end{enumerate}		
	\end{enumerate}
%	\item Sampling method
%	\begin{enumerate}
%		\item Effect of using only min for the loss or the top k samples, also applicable for black box method.
%		\item Priors on each of the patch covariances, in principle the same priors as in the black box model.
%		\item Blending the generated patches
%	\end{enumerate}
\end{enumerate}

Models with code implemented are accompanied by $^*$, $^\dagger$ results in~\cite{Yunchen2017Stein} for CIFAR-10, $^\circ$ results in~\cite{Yunchen2017Adversarial} for ImageNet, $^\ddagger$ results in~\cite{Yunchen2017Stein} or~\cite{Yunchen2017Adversarial} trained on MNIST.

Schedule for a total of 20-28 days:
\begin{enumerate}
	\item Fix aliasing issues in CelebA
	\item Add all layers of decoder as input for $\bSigma$ network
	\item Implement inverse Gamma for the EigDiag model, loss is the log likelihood of the Gamma distribution (1-2 days)
	\item Implement filtering (1-2 days)
	\item Test filtering with basis functions (1-2 days)
	\item Implement inverse Gamma for black box model (1-2 days)
	\item Extend to RGB images, use a linear transformation (multiplier and scale of [batch size, batch size]) (2-3 days)
	\item Implement normality test for black box model, losses~\ref{eq:L2} and~\ref{eq:L4} (1 day)
	\item Test on CelebA small with full model and large with black box model
	\item Test on Cifar-10 (1-2 days)
	\item Test on tiny image-net (2-3 days) 
	\item Retrain previous work methods (3-4 days)
	\item Write up (a week)
\end{enumerate}


==> figures/celeba_samples.tex <==
\def\plotw{0.24\linewidth}

% The images to show on each column
\def\1img{0}
\def\2img{15}
\def\3img{19}

\begin{figure}[t!]%[btph]
	\centering
	\setlength{\tabcolsep}{1pt} % Reduce spacing between the column
	\begin{tabular}{cccc}
	\includegraphics[width=\plotw]{img/celeba/sample_fig/sample/\1img} &
	\includegraphics[width=\plotw]{img/celeba/sample_fig/joint_samples/0/\1img} &
	\includegraphics[width=\plotw]{img/celeba/sample_fig/joint_samples/1/\1img} &
	\includegraphics[width=\plotw]{img/celeba/sample_fig/joint_samples/2/\1img} \\
	\includegraphics[width=\plotw]{img/celeba/sample_fig2/sample/\2img} &
	\includegraphics[width=\plotw]{img/celeba/sample_fig2/joint_samples/0/\2img} &
	\includegraphics[width=\plotw]{img/celeba/sample_fig2/joint_samples/1/\2img} &
	\includegraphics[width=\plotw]{img/celeba/sample_fig2/joint_samples/2/\2img} \\
	\includegraphics[width=\plotw]{img/celeba/sample_fig/sample/\3img} &
	\includegraphics[width=\plotw]{img/celeba/sample_fig/joint_samples/0/\3img} &
	\includegraphics[width=\plotw]{img/celeba/sample_fig/joint_samples/1/\3img} &
	\includegraphics[width=\plotw]{img/celeba/sample_fig/joint_samples/2/\3img} \\
	\end{tabular}
	\caption{ Samples drawn from our model.
	Our approach is able to generate structured residual samples from the latent variables.}
	\label{fig:celeba_samples}
\end{figure}

==> figures/celeba_sampling_eigvec.tex <==
\begin{figure}[t!]%[btph]
	\centering
	\setlength{\tabcolsep}{1pt} % Reduce spacing between the column
	\begin{tabular}{ccccc}
	{\small Input } & {\small AE} & {\small VAE} & {\small Ours 1} & {\small Ours 100} \\
	\includegraphics[width=0.24\linewidth]{img/kernel3x3} & & & 
	\end{tabular}
	\caption{ Sampling with a reduced number of eigen vectors in the covariance matrix.}
	\label{fig:celeba_sampling_eigvec}
\end{figure}

==> other_estimation_methods.tex <==
\subsection{Eigendecomposition}
\label{sec:eigen_decomposition}
One way to reduce the number of parameters that must be estimated is employing an eigendecomposition, where $\bLambda = \mathbf{Q} \mathbf{V} \mathbf{Q}^T$.
The matrix $\mathbf{Q}$ is an orthogonal, where each column is an eigenvector and $\mathbf{V}$ is a diagonal matrix with strictly positive eigenvalues.
An approximated precision matrix can be modeled by keeping only the the $n_v$ largest eigenvalues and their corresponding eigenvectors, such that $\bhLambda = \hat{\mathbf{Q}} \hat{\mathbf{V}} \hat{\mathbf{Q}}^T$.
The square root of the covariance is trivial to compute $\bM = \hat{\mathbf{Q}} \hat{\mathbf{V}}^{-\frac{1}{2}} \hat{\mathbf{Q}}^T = \bM^T$, and so it is the log determinant $\log(|\bhSigma|) = - \sum^{n_v}_{i=0}\log(\hat{v}_{ii})$.
The covariance matrix can be obtained by inverting the eigenvalue matrix $\bhSigma = \hat{\mathbf{Q}} \hat{\mathbf{V}}^{-1} \hat{\mathbf{Q}}^T$.
However, this is only a pseudo-inverse as the largest eigenvalues in $\bSigma$ were set to zero in the approximation step.

As stated above, $\hat{\mathbf{V}}$ must be positive and $\hat{\mathbf{Q}}$ must be an orthogonal matrix  to guarantee that $\bhSigma$ is symmetric and positive-definite.
The former can be easily achieved by having the network predict the $\log(\hat{\mathbf{V}})$, and the later with an additional orthogonality loss $|| \hat{\mathbf{Q}}^{T}\hat{\mathbf{Q}} - \bI||^2$.

%The number of eigenvectors that are required to have a good model of $\bLambda$ is in general too large to be practical.

%As stated above the $\log(|\bhSigma|)$ term is the sum of the eigenvalues, this term acts as a regularizer and it avoids the trivial solution of collapsing $\bLambda$ to zero, as a $\bLambda$ close to zero would have a $\bSigma$ with large eigenvalues.
%However, when estimating $\bhLambda$ with a small number of eigenvalues, 

\subsection{Eigendecomposition with diagonal}
\label{sec:eigen_decomposition_with_diagonal}
The eigendecomposition can be extended by adding a diagonal term $\bhLambda = \hat{\mathbf{Q}} \hat{\mathbf{V}} \hat{\mathbf{Q}}^T + a\bI$, where $a$ is a positive scalar.
This allows the network to model more complex matrices using the same number of eigenvectors, and it also ensures that the estimated matrices are invertible.

The log determinant is computed as $\log(|\bhSigma|) = - 2 \sum^n_i \log(\hat{l}_{ii})$ using the Cholesky decomposition $\bhLambda = \bhL \bhL^T$.
The covariance matrix $\bhSigma$ can still be easily computed using the Woodbury identity if $n >> n_v$ as it requires a matrix inversion the size of $n_v \times n_v$, 5 matrix multiplications and summing 2 matrices.
For sampling a Cholesky decomposition on $\bhSigma = \bhM \bhM^T$ can be used, or solving the system of equations $\bL^T \mathbf{y}^T = \mathbf{u}^T$.

In this setting, it matters whether the network is estimating the covariance or the precision as $(\hat{\mathbf{Q}} \hat{\mathbf{V}} \hat{\mathbf{Q}}^T  + a\bI)^{-1} \neq (\hat{\mathbf{Q}} \hat{\mathbf{V}} \hat{\mathbf{Q}}^T)^{-1}  + (a\bI)^{-1}$.
In the case of the covariance estimation $\bhSigma = \hat{\mathbf{Q}} \hat{\mathbf{V}} \hat{\mathbf{Q}}^T  + a\bI$, the sampling uses again the Cholesky decomposition $\bhSigma = \bhM \bhM^T$.
The log determinant is evaluated as $\log(|\bhSigma|) = 2 \sum^n_i \log(\hat{m}_{ii})$, and the precision matrix $\bhLambda$ can be computed with the Woodbury identity.

For both cases the same positive-definite constrains described section~\ref{sec:eigen_decomposition} can be employed, as the sum of positive-definite matrices is positive-definite, and the inverse is also positive-definite.

\subsection{Black box estimation}
\label{sec:black_box_estimation}

To be able to estimate the covariance matrix for large-dimensional data, an approach where we do not explicitly model $\bSigma$ is advantageous, as the size of the matrices is the order of $n^2$, where $n$ is the number of dimensions.

The square error term in the log likelihood $\br \bLambda \br^T$ can be expressed using a matrix decomposition as $\br \bL \bL^T \br^T$, where $\br = \bx - \bhx$ is the residual.
In a trained model, the learned multivariate Gaussian distribution should be able to produce the observed residual as a sample $\br \sim \mathcal{N}(\mathbf{0}, \bSigma)$ and precision should whiten the residual $\br \bL \sim \mathcal{N}(\mathbf{0}, \bI)$.

The covariance sampling and the whitening process can be modeled with neural networks 
\begin{align}
f_\bSigma(\bz, \bs) &\approx \bs \bM^T \sim \mathcal{N}(\mathbf{0}, \bSigma), \\
f_\bLambda(\bz, \br) &\approx \br \bL \sim \mathcal{N}(\mathbf{0}, \bI),
\end{align}
where $\bz$ is the low-dimensional representation of the input, $\bs \sim \mathcal{N}(\mathbf{0}, \bI))$ is a random sample, and the parameters of $f_\bSigma$ and $f_\bLambda$ are $\bpsi$ and $\boldsymbol{\gamma}$ respectively.

To train the parameters of these functions, the two steps iterative approach described in section~\ref{sec:new_model} is used.
As equation~\ref{eq:loss_nll_covariance} is being minimized, all the terms in the loss must be expressed using the the aforementioned whitening and sampling operations.
The squared error term $\br \bLambda \br^T$ can be computed as
\begin{equation}
L_1 = || f_{\Lambda}(\bz, \br) ||^2_2 \label{eq:L1}.
\end{equation}

The log determinant is more problematic as it cannot be evaluated directly, instead a set of functions are used as an approximation
\begin{align}
L_2 &= D_{KL}( f_{\Lambda}(\bz, f_{\Sigma}(\bz, \bs)) || \mathcal{N}(0, 1)), \label{eq:L2} \\
L_3 &= \argmin_{\bt_i \in \mathbf{T} } || \br - f_{\Sigma}(\bz, \bt_i) ||_2^2, \label{eq:L3} \\
L_4 &= D_{KL}(f_{\Lambda}(\bz, \br)||\mathcal{N}(0, 1)), \label{eq:L4}
\end{align}
where $\textbf{T}$ is a finite set of samples $\bt_i \sim \mathcal{N}(\mathbf{0}, \bI)$.
In eq.~\ref{eq:L2}, $f_{\Lambda}$ is forced to be the inverse of $f_{\Sigma}$.
Equation~\ref{eq:L3} ensures that $f_{\Sigma}$ is able to produce samples that closely resemble the residual $\br$.
The loss in eq.~\ref{eq:L4} encourages $f_{\Lambda}$ to whiten the residual $\br$.

Note that the KL divergence treats the vector output of the $f_{\Lambda}$ functions as set of samples from the one-dimensional distribution  $\mathcal{N}(0, 1)$.
The assumption in loss~\ref{eq:L2} is that $\bM^T$ is the inverse of $\bL$.
Writing the equation out $f_{\Lambda}(\bz, f_{\Sigma}(\bz, \bs)) \approx \bs\bM^T\bL$.
Therefore, we are restricting the type of matrices that can be modelled by the networks to symmetric square roots of $\bSigma$.

The optimization can be constrained further by using a deterministic version of loss~\ref{eq:L2} and its inverse
\begin{align}
L_5 & = || f_{\Lambda}(\bz, f_{\Sigma}(\bz, \bs)) - \bs ||_2^2, \label{eq:L5} \\
L_6 & = || f_{\Sigma}(\bz, f_{\Lambda}(\bz, \br)) - \br||_2^2, \label{eq:L6} \\
L_7 & = || f_{\Lambda}(\bz, \br) - \bt_{\max} ||_2^2, \label{eq:L7}
\end{align}
where $\bt_{\max}$ is the best sample $\bt_i$ from eq.~\ref{eq:L3}.
The first two losses penalize the functions if the are not the inverse of each other.
The loss in eq.~\ref{eq:L6} ensures that $f_{\Lambda}$ generates the same whiten image $\bt_{\max}$ that $f_{\Sigma}$ takes as input to produce $\br$, which ensures invertibility for the the best sample.

The final loss is 
\begin{equation}
L = \alpha_1 L_1 + \alpha_2 L_2 + \alpha_3 L_3 + \alpha_4 L_4,
\end{equation}
where $\alpha_i$ is a scalar weighting for each individual loss.

To summarize, the squared error error term is represented in $L_1$.
The log determinant is implicitly encoded in the interactions between the losses.
Namely, $f_{\Sigma}$ must be as simple as possible to minimize the effort that $f_{\Lambda}$ must do in $L_2$ to invert $f_{\Sigma}$, yet it has to be complex enough to capture the residual distribution in $L_3$.
Finally, $L_4$ encourages $f_{\Lambda}$ to minimize the square error by whitening $\br$.

\subsection{Sampling patch-based estimation}
\label{sec:patch_based_estimation}

The covariance matrices can be learnt with a sampling, where we still have a explicit representation of the covariance.

To train the model only loss~\ref{eq:L3} is needed, as by construction the model is generating valid covariance matrices.
Using this loss instead of the full negative log likelihood ensures that the covariance model is trying to learn a useful representation of the residuals.
For the VAE the loss in~\ref{eq:loss_nll_vae_iterative} is used.

To scale this approach to large images a patch-based approach can be used.
However, with this is not clear how to compute the log determinant of $\bSigma$ nor the precision matrix, as it is not trivial how to build a covariance matrix from a set of covariance patches.
Options for this include blending the covariances or generating a number of samples from the covariance and blending the best results in image space.

==> rebuttal/figures/celeba_samples_cherry_pick.tex <==
\def\plotw{0.225\linewidth}

\def\1img{15}
\def\2img{827}
\def\3img{222}
\def\4img{1560}
\def\5img{1450}

\begin{figure}[t!]%[btph]
	\centering
	\setlength{\tabcolsep}{1pt} % Reduce spacing between the column
	\begin{tabular}{ccccc}
	{$\bmu$} & 
	\includegraphics[align=c,width=\plotw]{img/celeba/sample_cov_sample_rebuttal0/sample/\1img} &
	\includegraphics[align=c,width=\plotw]{img/celeba/sample_cov_sample_rebuttal0/sample/\2img} &
	\includegraphics[align=c,width=\plotw]{img/celeba/sample_cov_sample_rebuttal0/sample/\3img} &
	\includegraphics[align=c,width=\plotw]{img/celeba/sample_cov_sample_rebuttal0/sample/\4img} \\[23pt]
	{\small Ours} & 
	\includegraphics[align=c,width=\plotw]{img/celeba/sample_cov_sample_rebuttal0/joint_samples/0/\1img} &
	\includegraphics[align=c,width=\plotw]{img/celeba/sample_cov_sample_rebuttal0/joint_samples/0/\2img} & 
	\includegraphics[align=c,width=\plotw]{img/celeba/sample_cov_sample_rebuttal0/joint_samples/0/\3img} & 
	\includegraphics[align=c,width=\plotw]{img/celeba/sample_cov_sample_rebuttal0/joint_samples/0/\4img} \\[23pt]
	\end{tabular}
	\caption{ Samples from the model for the CelebA dataset with a VAE with $\lambda = 1$, where $\bmu$ is the VAE sample and ours is $\bmu + \bepsilon$, where $\bepsilon$ is a sample from the predicted covariance.}
	\label{fig:celeba_samples_cherry_pick}
	\vspace{-0.2em}
\end{figure}

==> rebuttal/figures/cifar10_reconstructions.tex <==
 \def\plotw{0.12\linewidth}

% The images to show on each column
\def\1img{21}
\def\2img{57}
\def\3img{60}
\def\4img{11}
\def\5img{12}
\def\6img{13}
\def\7img{31}

\begin{figure}[t!]%[btph]
	\centering
	\setlength{\tabcolsep}{1pt} % Reduce spacing between the column
	\begin{tabular}{cccccccc}
	{\small Input }  & 
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/input/\1img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/input/\2img} &		
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/input/\3img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/input/\4img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/input/\5img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/input/\6img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/input/\7img}
	\\[9pt]
	{$\bmu$} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/cov/recons/\1img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/cov/recons/\2img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/cov/recons/\3img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/cov/recons/\4img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/cov/recons/\5img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/cov/recons/\6img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/cov/recons/\7img}
	\\[9pt]
	{\small Diag.} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/vae/best_recons/1/\1img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/vae/best_recons/1/\2img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/vae/best_recons/1/\3img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/vae/best_recons/1/\4img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/vae/best_recons/1/\5img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/vae/best_recons/1/\6img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/vae/best_recons/1/\7img}
	\\[9pt]
	{\small Ours} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/cov/best_recons/1/\1img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/cov/best_recons/1/\2img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/cov/best_recons/1/\3img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/cov/best_recons/1/\4img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/cov/best_recons/1/\5img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/cov/best_recons/1/\6img} &
	\includegraphics[align=c,width=\plotw]{img/cifar10/recons_fig/cov/best_recons/1/\7img}
	\\[11pt]
	\end{tabular}
	\caption{Comparison of image reconstructions on the CIFAR10 dataset, where $\bmu$ is a reconstruction from a VAE, Diag. is $\bmu + \bepsilon$, where $\bepsilon$ is a sample from a diagonal covariance matrix, and in our method $\bepsilon$ is a sample from a dense covariance matrix.} % (shown), and it is able to produce better reconstructions when taking more samples, results shown in the appendix.}
	\label{fig:cifar10_reconstructions}
	\vspace{-1.1em}
\end{figure}

%& {\small AE} & {\small AE-Ours} & {\small VAE} & {\small VAE-Ours}
